Doctor Recommendation in Online Health Forums via Expertise Learning

Huge volumes of patient queries are daily generated on online health forums, rendering manual doctor allocation a labor-intensive task. To better help patients, this paper studies a novel task of doctor recommendation to enable automatic pairing of a patient to a doctor with relevant expertise. While most prior work in recommendation focuses on modeling target users from their past behavior, we can only rely on the limited words in a query to infer a patient's needs for privacy reasons. For doctor modeling, we study the joint effects of their profiles and previous dialogues with other patients and explore their interactions via self-learning. The learned doctor embeddings are further employed to estimate their capabilities of handling a patient query with a multi-head attention mechanism. For experiments, a large-scale dataset is collected from Chunyu Yisheng, a Chinese online health forum, where our model exhibits the state-of-the-art results, outperforming baselines only consider profiles and past dialogues to characterize a doctor.

==> sections/error_analysis.tex <==
\subsection{Error Analysis}


We carefully inspect all experiment cases and observe error mainly occurred in two aspects: failure of recommendation within the same clinic and across various clinics. We sampled two cases to illustrate the causes of these two kinds of failures.


\input{tables/err_case_1}

\paragraph{False Recommendation in Same Clinic.}

Table \ref{tab:err_case_1} shows a query $q$ that doctor $D_1$ should be recommended while our model actually recommends doctor $D_2$. 
By examining doctor $D_1$ and doctor $D_2$, we observe that they are both ophthalmologists, and their profiles $p_1$ and $p_2$ are of similar lengths and details.
However, we observe doctor $D_1$ had only 30 history dialogues compared to doctor $D_2$'s 100 dialogues. 

As a result, the multi-head attention mechanism would not function for encoding doctor $D_1$ as well as for doctor $D_2$. 
Therefore, the model would tend to recommend doctor $D_2$ due to the rich dialogue contribution apart from profile.

This indicates a potential improvement of the existing encoding method. It is inevitable in practice that doctors have diverse serving experience. To get rid of the bias toward those doctors with more dialogue records, data augmentation \cite{zhang-etal-2020-parallel} could be adopted to enrich history of the doctors with less experience while with equivalent expertise. 
Based on sparse dialogues of one particular doctor and dialogues of other doctors with similar specialty in the same clinic, we could obtain virtual while reasonable dialogue ``history'' for the doctor with relatively less experience. It should help prevent recommendation preference to those doctors with fairly massive dialogues and further enhance recommendation performance.


\input{tables/err_case_2}

\paragraph{False Recommendation across Clinics.}

Table \ref{tab:err_case_2} shows a query $q$ recommended doctor $D_1$ by the forum while doctor $D_2$ by our model. Different from situation of the last case, doctor $D_1$ is a dermatovenereologist while $D_2$ an ophthalmologist. Intuitively, the symptom mentioned in $q$ is more likely to belong to dermatovenereology. The query also frequently refers to the keyword \textit{eye}, though, misleading the model's attention to focus on the affected part rather than illness itself. This phenomenon reveals that regarding queries with ambiguous information, our model sometimes attends to the less crucial message thus could recommend a doctor in another appropriate clinic.

To enhance our model in this aspect, topic model \cite{isonuma-etal-2020-tree} could be adopted to pre-classify doctors and queries into appropriate clinic. By clustering topics, it should be capable of reducing the possibility of cross-clinic recommendation. Additionally, we could further make use of the extracted topics to narrow down the scope of doctor candidates within the same clinic.

==> tables/case1_apd_att.tex <==
\begin{table}[h!]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|cl|}
\hline

\textbf{Head} $i$ &\textbf{Top 5 Keywords}\\

\hline
\hline

% attention regarding keyword "muscle"
\textsc{1}
&\tabincell{l}{瘙痒、湿疹、红肿、刺激、疱疹\\
(pruritus, eczema, redness and swelling,\\
irritation, herpes)}\\
\hline

% general attention
\textsc{2}
&\tabincell{l}{瘙痒、脱皮、传染、皮癣、细菌\\
(pruritus, desquamation, infection, ringworm,\\
bacteria)}\\
\hline

% attention regarding keyword "muscle"
\textsc{3}
&\tabincell{l}{过敏，红肿，皮炎，瘙痒，药膏\\
(allergy, redness and swelling, dermatitis,\\
pruritus, ointment)}\\
\hline

% attention regarding keyword "insomnia" and "wake up"
\textsc{4}
&\tabincell{l}{红肿，皮炎，痤疮，伤疤，粉刺\\
(redness and swelling, dermatitis, acne, scar,\\
pimple)}\\
\hline

% attention regarding keyword "muscle" and ”cervical vertebrae"
% a little general as well
\textsc{5}
&\tabincell{l}{脱皮，开裂，瘙痒，红斑，感染\\
(desquamation, chap, pruritus, erythema,\\
infection)}\\
\hline

% attention regarding keyword "muscle" and "cervical vertebrae"
\textsc{6}
&\tabincell{l}{瘙痒，性病，传染，疱疹，尖锐湿疣\\
(pruritus, venereal disease, infection, herpes,\\
condyloma acuminatum)}\\

\hline
\end{tabular}
%}
\end{center}
% \vspace{-0.5em}
\caption{The top 5 medical terms attended by each head given the input sample in \Cref{tab:case1_apd_texts}. The medical terms are from the THUOCL lexicon used in Section \ref{sec:dataset}.}
\label{tab:case1_apd_att}
%\vspace{0.5cm}
\end{table}

==> tables/case2_apd_att.tex <==
\begin{table}[h!]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|cl|}
\hline

\textbf{Head} $i$ &\textbf{Top 5 Keywords}\\

\hline
\hline

% attention regarding keyword "muscle"
\textsc{1}
&\tabincell{l}{怀孕，生理，月经，性行为，排卵期\\
(pregnancy, physiology, menstruation, sexual\\
behaviour, ovulation)}\\
\hline

% general attention
\textsc{2}
&\tabincell{l}{炎症，白带，阴道，宫颈，分泌物\\
(inflammation, leukorrhea, vagina, cervix\\
uteri, secreta)}\\
\hline

% attention regarding keyword "muscle"
\textsc{3}
&\tabincell{l}{性行为，预防措施，避孕药，艾滋，精子\\
(sexual behaviour, precaution, contraceptive,\\
AIDS, sperm)}\\
\hline

% attention regarding keyword "insomnia" and "wake up"
\textsc{4}
&\tabincell{l}{月经，激素，子宫内膜，出血，避孕药\\
(menstruation, hormone, endometrium,\\
bleeding, contraceptive)}\\
\hline

% attention regarding keyword "muscle" and ”cervical vertebrae"
% a little general as well
\textsc{5}
&\tabincell{l}{月经，怀孕，性行为，排卵期，流产\\
(menstruation, pregnancy, sexual behaviour,\\
ovulation, abortion)}\\
\hline

% attention regarding keyword "muscle" and "cervical vertebrae"
\textsc{6}
&\tabincell{l}{增生，肿块，卵巢，痛经，宫颈\\
(hyperplasia, lump, ovary, dysmenorrhea,\\
cervix uteri)}\\

\hline
\end{tabular}
%}
\end{center}
% \vspace{-0.5em}
\caption{The top 5 medical terms attended by each head given the input sample in \Cref{tab:case2_apd_texts}. The medical terms are from the THUOCL lexicon used in Section \ref{sec:dataset}.}
\label{tab:case2_apd_att}
%\vspace{0.5cm}
\end{table}

==> tables/case2_apd_texts_a.tex <==
\begin{table}[h]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|l|}
\hline
%\textbf{Query $q$}
\tabincell{l}{\textbf{Query $q$ from Anonymous Patient $P$}\\
There is brown secreta after my last menstruation, and it\\
disappears after sex. What’s wrong with me?}\\
\hline
\hline
\tabincell{l}{\textbf{Profile $p$ of Doctor $D$}\\
30 years of experience in obstetrics and gynecology.}\\
\hline
\hline
\tabincell{l}{\textbf{Attended Dialogue $d_1$}\\
$u_P$: The urine test result for pregnancy is negative for the\\
24th day after my last sexual behaviour, and it is the same\\
for the 20th, 22nd, 23rd. Can I rule out pregnancy?\\
$u_P$: I took contraceptive pill last month. I don’t know my\\
current ovulation.\\
$u_D$: Not pregnant, don’t worry.\\
$u_P$: I've been getting yellowish vaginal discharge lately.\\
Am I inflamed?\\
$u_D$: It’s fungal vaginitis. I suggest you take fluconazole\\
pills.}\\
\hline
\tabincell{l}{\textbf{Attended Dialogue $d_2$}\\
$u_P$: My boyfriend and I had sex with condom. It was the\\
first time for me, but my boyfriend had had sex life with\\
others. Is there a high chance I get infected with HPV?\\
$u_D$: From your description, it is not likely to happen.}\\
\hline
\tabincell{l}{\textbf{Attended Dialogue $d_3$}\\
$u_P$: My period has been lasting for 8 days. I bleed a lot\\
and have blood clots. What’ the matter with me?\\
$u_P$: In the past year my period has always been regular.\\
But in the past two months I took Ejiao for a few days.\\
$u_D$: It’s abnormal and it could be caused by Ejiao. I\\
suggest hemostasis, or it could lead to anemia.}\\
\hline
\tabincell{l}{\textbf{Attended Dialogue $d_4$}\\
$u_P$: My vaginal opening is like white petal. I have had\\
sexual experience, but I feel alright. Is it condyloma\\
acuminatum?\\
$u_D$: How long has this lasted? How are you feeling?\\
$u_P$: I feel nothing.\\
$u_D$: It’s normal, not condyloma acuminatum. It is likely\\
to be hymen residue.}\\
\hline
\end{tabular}
%}
\end{center}
\vspace{-1em}
\caption*{(a)}
\end{table}

==> tables/case2_apd_texts_b.tex <==
\begin{table}[h]\small

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|cl|}
\hline

\textbf{Head} $i$ &\textbf{Top 5 Keywords}\\

\hline
\hline

% attention regarding keyword "muscle"
\textsc{1}
&\tabincell{l}{怀孕，生理，月经，性行为，排卵期\\
(pregnancy, physiology, menstruation, sexual\\
behaviour, ovulation)}\\
\hline

% general attention
\textsc{2}
&\tabincell{l}{炎症，白带，阴道，宫颈，分泌物\\
(inflammation, leukorrhea, vagina, cervix\\
uteri, secreta)}\\
\hline

% attention regarding keyword "muscle"
\textsc{3}
&\tabincell{l}{性行为，预防措施，避孕药，艾滋，精子\\
(sexual behaviour, precaution, contraceptive,\\
AIDS, sperm)}\\
\hline

% attention regarding keyword "insomnia" and "wake up"
\textsc{4}
&\tabincell{l}{月经，激素，子宫内膜，出血，避孕药\\
(menstruation, hormone, endometrium,\\
bleeding, contraceptive)}\\
\hline

% attention regarding keyword "muscle" and ”cervical vertebrae"
% a little general as well
\textsc{5}
&\tabincell{l}{月经，怀孕，性行为，排卵期，流产\\
(menstruation, pregnancy, sexual behaviour,\\
ovulation, abortion)}\\
\hline

% attention regarding keyword "muscle" and "cervical vertebrae"
\textsc{6}
&\tabincell{l}{增生，肿块，卵巢，痛经，宫颈\\
(hyperplasia, lump, ovary, dysmenorrhea,\\
cervix uteri)}\\

\hline
\end{tabular}
%}
\end{center}
\vspace{-1em}
\caption*{(b)}
% \caption{The top 5 medical terms attended by each head given the input sample in \Cref{tab:case2_apd_texts}. The medical terms are from the THUOCL lexicon used in Section \ref{sec:dataset}.}
% \label{tab:case2_apd_att}

\caption{The sample patient query $q$ from anonymous patient $P$ on the top, followed by the profile of a sample doctor $D$ and four dialogues $D$ engaged before. $u_P$ refers to utterances of $P$, and $u_D$ utterances of $D$. (b) The top 5 medical terms attended by each head given the input sample in \Cref{tab:case2_apd_texts}(a). The medical terms are from the THUOCL lexicon in Section \ref{sec:dataset}.}
% \protect\footnotemark
\label{tab:case2_apd_texts}
% \vspace{0.2cm}
\end{table}
% \footnotetext{We omit the original Chinese text and abbreviate the dialogues for the sake of readability.}

==> tables/err_case_1.tex <==
\begin{table}[ht]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{c|l}
\hline

\textsc{$q$}
&\tabincell{l}{小孩子经常眨眼，使劲连续眨那种，有过敏性鼻\\炎。请问这个是什么情况啊？
\\(The kid often blinks hard and continuously, and it\\hasallergic-rhinitis. What's the kid's problem?)}\\
\hline
\hline

\textsc{$p_1$}
&\tabincell{l}{屈光不正，弱视，斜视，结膜炎，麦粒肿等眼病\\的诊断和治疗
\\(Good at diagnosing and treating ophthalmocace\\including refractive error, amblyopia, strabismus,\\conjunctivitis, hordeolum, and the like.)}\\
\hline

\textsc{$p_2$}
&\tabincell{l}{眼科疾病的诊治，白内障，屈光不正，眼底病，\\眼表疾病等常见疾病的诊断治疗
\\(Good at diagnosing and treating ophthalmocace\\including  cataract，refractive error，ocula fundus\\diseases，ocular surface diseases, and the like.)}\\

\hline

\end{tabular}
%}
\end{center}
% \vspace{-0.5em}
\caption{Case 1: failure of recommendation within the same clinic. To highlight key information, we remove some tokens without altering main semantics.}
\label{tab:err_case_1}
% \vspace{-0.5em}
\end{table}

==> tables/err_case_2.tex <==
\begin{table}[ht]\small
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\begin{center}
%\resizebox{0.99\textwidth}{!}{
\begin{tabular}{c|l}
\hline

\textsc{$q$}
&\tabincell{l}{小朋友眼皮上长了一片小疙瘩，眼皮就变得有点\\粗糙，咋办？
\\(There is a stretch of small pimples on the kid's\\eyelid, making it a little coarse. What should we\\do?)}\\
\hline
\hline

\textsc{$p_1$}
&\tabincell{l}{痤疮，敏感性皮肤，激素依赖性皮炎，玫瑰痤\\疮，荨麻疹等皮肤病的治疗
\\(Good at treating skin condition including acne,\\skin allergy, hormone dependence dermatitis,\\rosacea, urticaria, and the like.)}\\
\hline

\textsc{$p_2$}
&\tabincell{l}{眼科疾病的诊治，青光眼，白内障，屈光不正，\\眼底病，眼表疾病等常见疾病的诊断治疗
\\(Good at diagnosing and treating ophthalmocace\\including glaucoma, cataract，refractive error,\\ocular fundus diseases，ocular surface diseases,\\and the like.)}\\

\hline

\end{tabular}
%}
\end{center}
% \vspace{-0.5em}
\caption{Case 2: failure of recommendation across clinics. To highlight key information in profile $p_1$, we remove some tokens indicating other diseases.}
\label{tab:err_case_2}
% \vspace{-0.5em}
\end{table}
